MPRNet: Multi-Path Residual Network for Lightweight Image Super Resolution

Lightweight super resolution networks have extremely importance for real-world applications. In recent years several SR deep learning approaches with outstanding achievement have been introduced by sacrificing memory and computational cost. To overcome this problem, a novel lightweight super resolution network is proposed, which improves the SOTA performance in lightweight SR and performs roughly similar to computationally expensive networks. Multi-Path Residual Network designs with a set of Residual concatenation Blocks stacked with Adaptive Residual Blocks: ($i$) to adaptively extract informative features and learn more expressive spatial context information; ($ii$) to better leverage multi-level representations before up-sampling stage; and ($iii$) to allow an efficient information and gradient flow within the network. The proposed architecture also contains a new attention mechanism, Two-Fold Attention Module, to maximize the representation ability of the model. Extensive experiments show the superiority of our model against other SOTA SR approaches.

==> files/fig/more_BD.tex <==
\setlength\tabcolsep{4.5pt}
\begin{figure*}[]
\centering
\tiny
\scalebox{0.8}{
\begin{tabular}{ccccc}
\multirow{-9.510}{*}{\adjustbox{valign=b}{\includegraphics[width=.29\textwidth, height=4.24cm]{files/supplementry/BD_1/S_HR.png}}} 
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_1/HR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_1/bicubic.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_1/SRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_1/FSRCNN.png} \\
 & \small HR & \small Bicubic & \small SRCNN & \small FSRCNN \\
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_1/VDSR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_1/IRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_1/SRMDNF.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_1/ours.png} \\
 \small Urban100 -- img028 & \small VDSR & \small IRCNN\_G & \small SRMDNF & \small MPRNet (Ours) \\
 \vspace{1pt}
\end{tabular}}
% \vspace{-20pt}
% \noindent\makebox[\linewidth]{\rule{\textwidth}{1pt}} \\ 
\vspace{20pt}

\scalebox{0.8}{
\begin{tabular}{ccccc}
\multirow{-9.510}{*}{\adjustbox{valign=b}{\includegraphics[width=.29\textwidth, height=4.24cm]{files/supplementry/BD_2/S_HR.png}}} 
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_2/HR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_2/bicubic.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_2/SRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_2/FSRCNN.png} \\
 & \small HR & \small Bicubic & \small SRCNN & \small FSRCNN \\
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_2/FSRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_2/IRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_2/SRMDNF.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_2/ours.png} \\
 \small Urban100 -- img096 & \small VDSR & \small IRCNN\_G & \small SRMDNF & \small MPRNet (Ours) \\
 \vspace{1pt}
\end{tabular}}
\caption{Qualitative results on \textbf{BN} degradation model with a scale factor $\times$3.}
% \vspace{-20pt}
% \noindent\makebox[\linewidth]{\rule{\textwidth}{1pt}} \\ 
\vspace{20pt}

\scalebox{0.8}{
\begin{tabular}{ccccc}
\multirow{-9.510}{*}{\adjustbox{valign=b}{\includegraphics[width=.29\textwidth, height=4.24cm]{files/supplementry/DN_1/S_HR.png}}} 
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/DN_1/HRs.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/DN_1/bicubic.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/DN_1/FSRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/DN_1/VDSR.png} \\
 & \small HR & \small Bicubic & \small SRCNN & \small VDSR \\
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/DN_1/IRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/DN_1/SRMD.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/DN_1/RDN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/DN_1/ours06.png} \\
 \small Set14 -- img006 & \small IRCNN\_C & \small SRMD & \small RDN & \small MPRNet (Ours) \\
 \vspace{1pt}
\end{tabular}}
% \vspace{-20pt}
% \noindent\makebox[\linewidth]{\rule{\textwidth}{1pt}}
\vspace{20pt}

\scalebox{0.8}{
\begin{tabular}{ccccc}
\multirow{-9.510}{*}{\adjustbox{valign=b}{\includegraphics[width=.29\textwidth, height=4.24cm]{files/supplementry/DN_2/S_HR.png}}} 
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/DN_2/HR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/DN_2/LR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/DN_2/SRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/DN_2/VDSR.png} \\
 & \small HR & \small Bicubic & \small SRCNN & \small VDSR \\
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/DN_2/IRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/DN_2/SRMD.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/DN_2/RDN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/DN_2/ours.png} \\
 \small Set5 -- img003 & \small IRCNN\_C & \small SRMD & \small RDN & \small MPRNet (Ours) \\
 \vspace{1pt}
\end{tabular}}
% \vspace{-20pt}
\caption{Qualitative results on \textbf{DN} degradation model with a scale factor $\times$3.}
\label{tab:more}
\end{figure*}

==> files/fig/more_BI.tex <==
\setlength\tabcolsep{4.5pt}
\begin{figure*}[]
\centering
\tiny
% \scalebox{0.8}{
% \begin{tabular}{ccccc}
% \multirow{-9.510}{*}{\adjustbox{valign=b}{\includegraphics[width=.29\textwidth, height=4.24cm]{files/supplementry/BI_1/24_HR_full.png}}} 
%  & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_1/24_HR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_1/LR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_1/VDSR_24_SR_U100.JPG} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_1/MemNet_24_SR_U100.JPG} \\
%  & \small HR & \small Bicubic & \small VDSR & \small MemNet \\
%  & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_1/CARN_M_24_SR_U100.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_1/CARN_24_SR_U100.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_1/SRFBN-S_24_SR_U100.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_1/Ours_24_SR_100_[75,640].png} \\
%  \small Urban100 -- img024 & \small LapSRN & \small CARN & \small SRFBN-S & \small MPRNet (Ours) \\
%  \vspace{1pt}
% \end{tabular}}
% % \vspace{-20pt}
% % \noindent\makebox[\linewidth]{\rule{\textwidth}{1pt}} \\ 
% \vspace{20pt}

\scalebox{0.8}{
\begin{tabular}{ccccc}
\multirow{-9.510}{*}{\adjustbox{valign=b}{\includegraphics[width=.29\textwidth, height=4.24cm]{files/supplementry/BI_2/S_HR.png}}} 
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_2/HR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_2/LR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_2/FSRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_2/carn_m61.png} \\
 & \small HR & \small Bicubic & \small VDSR & \small MemNet \\
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_2/SRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_2/carn61.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_2/SRFBN-s61.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_2/our61.png} \\
 \small Urban100 -- img061 & \small LapSRN & \small CARN & \small SRFBN-S & \small MPRNet (Ours) \\
 \vspace{1pt}
\end{tabular}}
% \vspace{-20pt}
% \noindent\makebox[\linewidth]{\rule{\textwidth}{1pt}} \\ 
\vspace{20pt}

% \scalebox{0.8}{
% \begin{tabular}{ccccc}
% \multirow{-9.510}{*}{\adjustbox{valign=b}{\includegraphics[width=.29\textwidth, height=4.24cm]{files/supplementry/BI_3/S_HR.png}}} 
%  & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_3/HR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_3/LR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_3/SRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_3/memnet.png} \\
%  & \small HR & \small Bicubic & \small VDSR & \small MemNet \\
%  & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_3/carn_m19.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_3/carn19.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_3/SRFBN-s19.png} & \includegraphics[width=.15\textwidth,   height=1.94cm]{files/supplementry/BI_3/ours19.png} \\
%  \small Urban100 -- img019 & \small LapSRN & \small CARN & \small SRFBN-S & \small MPRNet (Ours) \\
%  \vspace{1pt}
% \end{tabular}}
% % \vspace{-20pt}
% % \noindent\makebox[\linewidth]{\rule{\textwidth}{1pt}}
% \vspace{20pt}

\scalebox{0.8}{
\begin{tabular}{ccccc}
\multirow{-9.510}{*}{\adjustbox{valign=b}{\includegraphics[width=.29\textwidth, height=4.24cm]{files/supplementry/BI_4/S_HR.png}}} 
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_4/HR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_4/LR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_4/SRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_4/FSRCNN.png} \\
 & \small HR & \small Bicubic & \small VDSR & \small MemNet \\
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_4/carn-m.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_4/carn.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_4/SRFBN-S.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BI_4/ours_85.png} \\
 \small Urban100 -- img085 & \small LapSRN & \small CARN & \small SRFBN-S & \small MPRNet (Ours) \\
 \vspace{1pt}
\end{tabular}}
% \vspace{-20pt}
\caption{Qualitative results on \textbf{BI} degradation model with a scale factor $\times$4 on $Urban100$ dataset.}
\label{tab:more}
% \vspace{10pt}
% \scalebox{0.8}{
% \begin{tabular}{ccccc}
% \multirow{-9.510}{*}{\adjustbox{valign=b}{\includegraphics[width=.29\textwidth, height=4.24cm]{files/supplementry/BD_1/S_HR.png}}} 
%  & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_1/HR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_1/bicubic.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_1/SRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_1/FSRCNN.png} \\
%  & \small HR & \small Bicubic & \small SRCNN & \small FSRCNN \\
%  & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_1/VDSR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_1/IRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_1/SRMDNF.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_1/ours.png} \\
%  \small Urban100 -- img028 & \small VDSR & \small IRCNN\_G & \small SRMDNF & \small MPRNet (Ours) \\
%  \vspace{1pt}
% \end{tabular}}
% % \vspace{-20pt}
% % \noindent\makebox[\linewidth]{\rule{\textwidth}{1pt}} \\ 
% \vspace{20pt}

% \scalebox{0.8}{
% \begin{tabular}{ccccc}
% \multirow{-9.510}{*}{\adjustbox{valign=b}{\includegraphics[width=.29\textwidth, height=4.24cm]{files/supplementry/BD_2/S_HR.png}}} 
%  & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_2/HR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_2/bicubic.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_2/SRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_2/FSRCNN.png} \\
%  & \small HR & \small Bicubic & \small SRCNN & \small FSRCNN \\
%  & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_2/FSRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_2/IRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_2/SRMDNF.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/supplementry/BD_2/ours.png} \\
%  \small Urban100 -- img096 & \small VDSR & \small IRCNN\_G & \small SRMDNF & \small MPRNet (Ours) \\
%  \vspace{1pt}
% \end{tabular}}
% \caption{Qualitative results on \textbf{BN} degradation model with a scale factor $\times$3 on $Urban100$ dataset.}
% % \vspace{-20pt}
% % \noindent\makebox[\linewidth]{\rule{\textwidth}{1pt}} \\ 
% \vspace{20pt}

\end{figure*}

==> files/fig/more_DN.tex <==
\setlength\tabcolsep{4.5pt}
\begin{figure*}[]
\centering
\tiny
\caption{More qualitative results on \textbf{DN} degradation dataset with scale factor $\times$4. $1^{st}$ from Set5; $2^{nd}$ from Set14; $3^{rd}$ from B100 ; $4^{th}$ from Urban100. }
\vspace{20pt}
\scalebox{0.9}{
\begin{tabular}{ccccc}
\multirow{-9.510}{**}{\adjustbox{valign=b}{\includegraphics[width=.29\textwidth, height=4.24cm]{files/pic/BI/S_HR.png}}} 
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/HR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/LR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/SRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/FSRCNN.png} \\
 & \small HR & \small Bicubic & \small SRCNN & \small FSRCNN \\
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/IRCNN_C-m.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/IRCNN_C.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/SRMD.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/ours.png} \\
 \small img011.94 from Urban100 & \small VDSR & \small IRCNN_C & \small SRMD & \small MPRNet(Ours) \\
 \vspace{1pt}
\end{tabular}}
% \vspace{-20pt}
% \noindent\makebox[\linewidth]{\rule{\textwidth}{1pt}} \\ 
\vspace{20pt}

\scalebox{0.9}{
\begin{tabular}{ccccc}
\multirow{-9.510}{*}{\adjustbox{valign=b}{\includegraphics[width=.29\textwidth, height=4.24cm]{files/pic/BI/S_HR.png}}} 
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/HR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/LR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/SRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/FSRCNN.png} \\
 & \small HR & \small Bicubic & \small SRCNN & \small FSRCNN \\
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/IRCNN_C-m.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/IRCNN_C.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/SRMD.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/ours.png} \\
 \small img011.94 from Urban100 & \small VDSR & \small IRCNN_C & \small SRMD & \small MPRNet(Ours) \\
 \vspace{1pt}
\end{tabular}}
% \vspace{-20pt}
% \noindent\makebox[\linewidth]{\rule{\textwidth}{1pt}} \\ 
\vspace{20pt}

\scalebox{0.9}{
\begin{tabular}{ccccc}
\multirow{-9.510}{*}{\adjustbox{valign=b}{\includegraphics[width=.29\textwidth, height=4.24cm]{files/pic/BI/S_HR.png}}} 
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/HR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/LR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/SRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/FSRCNN.png} \\
 & \small HR & \small Bicubic & \small SRCNN & \small FSRCNN \\
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/IRCNN_C-m.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/IRCNN_C.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/SRMD.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/ours.png} \\
 \small img011.94 from Urban100 & \small VDSR & \small IRCNN_C & \small SRMD & \small MPRNet(Ours) \\
 \vspace{1pt}
\end{tabular}}
% \vspace{-20pt}
% \noindent\makebox[\linewidth]{\rule{\textwidth}{1pt}}
\vspace{20pt}

\scalebox{0.9}{
\begin{tabular}{ccccc}
\multirow{-9.510}{*}{\adjustbox{valign=b}{\includegraphics[width=.29\textwidth, height=4.24cm]{files/pic/BI/S_HR.png}}} 
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/HR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/LR.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/SRCNN.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/FSRCNN.png} \\
 & \small HR & \small Bicubic & \small SRCNN & \small FSRCNN \\
 & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/IRCNN_C-m.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/IRCNN_C.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/SRMD.png} & \includegraphics[width=.15\textwidth, height=1.94cm]{files/pic/BI/ours.png} \\
 \small img011.94 from Urban100 & \small VDSR & \small IRCNN_C & \small SRMD & \small MPRNet(Ours) \\
 \vspace{1pt}
\end{tabular}}
% \vspace{-20pt}

\label{tab:more_DN}
\end{figure*}

==> files/supplementry/params.tex <==
\begin{table*}[]
\begin{adjustbox}{width=1\textwidth}
\setlength\arrayrulewidth{1.0pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline

 & Method & \begin{tabular}[c]{@{}c@{}}\textbf{LapSRN}{\cite{lai2017deep}}\\ \hline Params-MAC\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{VDSR}{\cite{kim2016accurate}}\\ \hline Params-MAC\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{MemNet}{\cite{tai2017memnet}} \\ \hline Params-MAC\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{CARN}{\cite{ahn2018fast}}\\ \hline Params-MAC\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{FALSR-A}{\cite{chu2019fast}}\\ \hline Params-MAC\end{tabular} & \begin{tabular}[c]{@{}c@{}} \textbf{SRMDNF}{\cite{tong2017image}}\\ \hline Params-MAC\end{tabular} & \begin{tabular}[c]{@{}c@{}} \textbf{SRDenseNet}{\cite{zhang2018learning}}\\ \hline Params-MAC\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{OISR-LF-s}{\cite{he2019ode}}\\ \hline Params-MAC\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{MSRN}{\cite{li2018multi}}\\ \hline Params-MAC\end{tabular} &\begin{tabular}[c]{@{}c@{}}\textbf{RDN}{\cite{zhang2018residual}}\\ \hline Params-MAC\end{tabular} &
 \begin{tabular}[c]{@{}c@{}}\textbf{MPRNet[Ours]}\\ \hline Params-MAC\end{tabular} \\ \hline \hline
Scale & \begin{tabular}[c]{@{}c@{}}$\times2$\\ $\times3$\\ $\times4$\end{tabular} & \begin{tabular}[c]{@{}c@{}}813K-29G\\ -----\\ 813K-149.4G\end{tabular} & \begin{tabular}[c]{@{}c@{}}665K-612.6G\\ 665K-612.6G\\ 665K-612.6G\end{tabular} & \begin{tabular}[c]{@{}c@{}}677K-2662.4G\\ 667K-2662.4G\\ 667K-2662.4G\end{tabular} & \begin{tabular}[c]{@{}c@{}}1592K-222.8G\\ 1592K-118.8G\\ 1592K-90.9G\end{tabular} & \begin{tabular}[c]{@{}c@{}}1021K-234.7G\\ -----\\ -----\end{tabular} & \begin{tabular}[c]{@{}c@{}}1513K-347.7G\\ 1530K-156.3G\\ 1555K-89.3G\end{tabular} & \begin{tabular}[c]{@{}c@{}}-----\\ -----\\ 2015K-389.9G\end{tabular} & \begin{tabular}[c]{@{}c@{}}1370K-316.2G\\ 1550K-160.1G\\ 1552K-114.2G\end{tabular} & \begin{tabular}[c]{@{}c@{}}5930K-1365.8G\\ 6008K-621.2G\\ 6033K-365.1G\end{tabular} &
\begin{tabular}[c]{@{}c@{}}22120K-5096.2G\\ 22310K-2281.2G\\ 2227K-1309.2G\end{tabular} &
\begin{tabular}[c]{@{}c@{}}\textbf{461K-106.2G}\\ \textbf{509.8K-66.1G}\\ \textbf{509.8K-29G}\end{tabular} \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Comparisons on the number of network parameters and MAC operations for all scale factors $[\times2, \times3, \times4]$ in detail (PSNR and SSIM are provided in the submitted manuscript).}
\label{tab:subparam}
\end{table*}

==> files/tables/Tabel_BI_M1.tex <==
\begin{table*}[ht!]
\caption{\small Comparison with costly methods (up to $6000K$ number of network parameters). Mean PSNR/SSIM values on scale factors $[\times2, \times3, \times4]$ with the \textbf{BI} degradation model. Best results are \textbf{highlighted} and second best results are \underline{underlined}.}
% \vspace{-5.0pt}
\begin{adjustbox}{width=1\textwidth}
\setlength\arrayrulewidth{1.0pt}
% \scalebox{0.6}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}\multirow{2}{*}{} \\ \hline Params-MAC \\ \hline Dataset \end{tabular} & \begin{tabular}[c]{@{}c@{}}\multirow{2}{*}{} \textbf{Models} \\ \hline $\times$4 \\ \hline Scale \end{tabular} & \begin{tabular}[c]{@{}c@{}}\multirow{2}{*}{}\textbf{DRCN} {\cite{kim2016deeply}} \\ \hline  1774K-17974G \\ \hline PSNR/SSIM \end{tabular} & \begin{tabular}[c]{@{}c@{}}\multirow{2}{*}{}\textbf{CARN} {\cite{ahn2018fast}}\\ \hline  1592K-90.9G \\ \hline PSNR/SSIM  \end{tabular} & \begin{tabular}[c]{@{}c@{}}\multirow{2}{*}{}\textbf{SRMD(NF)} {\cite{tong2017image}} \\ \hline  1555K-89.3G \\ \hline PSNR/SSIM \end{tabular} &
\begin{tabular}[c]{@{}c@{}}\multirow{2}{*}{}\textbf{SelNet} {\cite{choi2017deep}} \\ \hline  1417K-83.1G \\ \hline PSNR/SSIM \end{tabular} &
\begin{tabular}[c]{@{}c@{}}\multirow{2}{*}{}\textbf{SRDenseNet} {\cite{zhang2018learning}} \\ \hline 2015K-389.9G \\ \hline PSNR/SSIM \end{tabular} & \begin{tabular}[c]{@{}c@{}}\multirow{2}{*}{}\textbf{MoreMNAS-A} {\cite{chu2019multi}} \\ \hline 1039K-238.6G  \\ \hline PSNR/SSIM \end{tabular} &  \begin{tabular}[c]{@{}c@{}}\multirow{2}{*}{}\textbf{FALSR-A} {\cite{chu2019fast}} \\ \hline 1021K-234.7G \\ \hline PSNR/SSIM \end{tabular} &
\begin{tabular}[c]{@{}c@{}}\multirow{2}{*}{}\textbf{OISR-RK2-s} {\cite{he2019ode}} \\ \hline 1520K-114.2G \\ \hline PSNR/SSIM \end{tabular} &
\begin{tabular}[c]{@{}c@{}}\multirow{2}{*}{}\textbf{MSRN} {\cite{li2018multi}} \\ \hline 6078K-349.8G \\ \hline PSNR/SSIM \end{tabular}&  \begin{tabular}[c]{@{}c@{}}\multirow{2}{*}{}\textbf{MPRNet [Ours]} \\ \hline 509K-29.3G \\ \hline PSNR/SSIM \end{tabular} \\ \hline \hline
Set5 & \begin{tabular}[c]{@{}c@{}}$\times$2\\ $\times$3\\ $\times$4\end{tabular} & \begin{tabular}[c]{@{}c@{}}37.63/0.9588\\ 33.82/0.9226\\ 31.53/0.8854\end{tabular} & \begin{tabular}[c]{@{}c@{}}37.76/0.9590\\ 34.29/0.9255\\ 32.13/0.8937\end{tabular} & \begin{tabular}[c]{@{}c@{}}37.79/0.9600\\ 34.12/0.9250\\ 31.96/0.8930\end{tabular} & \begin{tabular}[c]{@{}c@{}}37.89/0.9598\\ 34.27/0.9257\\ 32.00/0.8931\end{tabular} &\begin{tabular}[c]{@{}c@{}}--------\\ --------\\ 32.02/0.8934\end{tabular}  &\begin{tabular}[c]{@{}c@{}}37.63/0.9584\\ --------\\ --------\end{tabular} &  \begin{tabular}[c]{@{}c@{}}37.82/0.9595\\ --------\\ --------\end{tabular}&
\begin{tabular}[c]{@{}c@{}}37.98/0.9604\\ \ul{34.39/0.9273}\\ \ul{32.21/0.8950}\end{tabular} &\begin{tabular}[c]{@{}c@{}} \textbf{38.08/0.9605}\\ 34.38/0.9262\\ 32.07/0.8903\end{tabular} & 
\begin{tabular}[c]{@{}c@{}} \ul{38.03/0.9610} \\ \textbf{34.40/0.9285}\\ \textbf{32.28/0.9034}\end{tabular} \\ \hline 
Set14 & \begin{tabular}[c]{@{}c@{}}$\times$2\\ $\times$3\\ $\times$4\end{tabular} & \begin{tabular}[c]{@{}c@{}}33.04/0.9118\\ 29.76/0.8311\\ 28.02/0.7670\end{tabular} & \begin{tabular}[c]{@{}c@{}}33.52/0.9166\\ 30.29/0.8407\\ 28.60/0.7806\end{tabular} & \begin{tabular}[c]{@{}c@{}}33.32/0.9150\\ 30.04/0.8370\\ 28.35/0.7770\end{tabular} & \begin{tabular}[c]{@{}c@{}}33.61/0.9160\\ 30.30/0.8399\\ 28.49/0.7783\end{tabular} &\begin{tabular}[c]{@{}c@{}}--------\\ --------\\ 28.50/0.7782\end{tabular} & \begin{tabular}[c]{@{}c@{}}33.23/0.9138\\ --------\\ --------\end{tabular} &  \begin{tabular}[c]{@{}c@{}}33.55/0.9168\\ --------\\ --------\end{tabular} &
\begin{tabular}[c]{@{}c@{}}33.58/0.9172\\ 30.33/0.8420\\ 28.63/0.7822\end{tabular} 
&\begin{tabular}[c]{@{}c@{}}\textbf{33.74/0.9170}\\ \ul{30.34/0.8395}\\ \ul{28.60/0.7751}\end{tabular} & 
\begin{tabular}[c]{@{}c@{}} \ul{33.63/0.9176} \\ \textbf{30.35/0.8419} \\ \textbf{28.62/0.7810} \end{tabular}\\ \hline 
B100 & \begin{tabular}[c]{@{}c@{}}$\times$2\\ $\times$3\\ $\times$4\end{tabular} & \begin{tabular}[c]{@{}c@{}}31.85/0.8942\\ 28.80/0.7963\\ 27.23/0.7233\end{tabular} & \begin{tabular}[c]{@{}c@{}}32.09/0.8978\\ 29.06/0.8434\\ 27.58/0.7349\end{tabular} & \begin{tabular}[c]{@{}c@{}}32.05/0.8980\\ 28.97/0.8030\\ 27.49/0.7340\end{tabular} &\begin{tabular}[c]{@{}c@{}}32.08/0.8984\\ 28.97/0.8022\\ 28.49/0.7783\end{tabular} &\begin{tabular}[c]{@{}c@{}}--------\\ --------\\ 27.53/0.7337\end{tabular} & \begin{tabular}[c]{@{}c@{}}31.95/0.8961\\ --------\\ --------\end{tabular} &  \begin{tabular}[c]{@{}c@{}}32.12/0.8987\\ --------\\ --------\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}32.18/0.8996\\ \ul{29.10/0.8083}\\ \ul{27.58/0.7364}\end{tabular} &
\begin{tabular}[c]{@{}c@{}}\textbf{32.23/0.9013}\\ 29.08/0.8041\\ 27.52/0.7273\end{tabular} &
\begin{tabular}[c]{@{}c@{}}\ul{32.22/0.9099}\\ \textbf{29.13/0.8175}\\ \textbf{27.60/0.7373}\end{tabular}\\ \hline 
Urban100 & \begin{tabular}[c]{@{}c@{}}$\times$2\\ $\times$3\\ $\times$4\end{tabular} & \begin{tabular}[c]{@{}c@{}}30.75/0.9133\\ 27.15/0.8276\\ 25.14/0.7510\end{tabular} & \begin{tabular}[c]{@{}c@{}}31.92/0.9256\\ 28.06/0.8493\\ 26.07/0.7837\end{tabular} & \begin{tabular}[c]{@{}c@{}}31.33/0.9200\\ 27.57/0.8400\\ 25.68/0.7730\end{tabular} &\begin{tabular}[c]{@{}c@{}}--------\\ --------\\ --------\end{tabular} &\begin{tabular}[c]{@{}c@{}}--------\\ --------\\ 26.05/0.7819\end{tabular} & \begin{tabular}[c]{@{}c@{}}31.24/0.9187\\ --------\\ --------\end{tabular} &  \begin{tabular}[c]{@{}c@{}}31.93/0.9256\\ --------\\ --------\end{tabular} &
\begin{tabular}[c]{@{}c@{}}32.21/0.8950\\ 28.03/0.8544\\ 26.14/0.7874\end{tabular} &
\begin{tabular}[c]{@{}c@{}}\ul{32.22/0.9326}\\ \ul{28.08/0.8554}\\ \ul{26.04/0.7896}\end{tabular} &\begin{tabular}[c]{@{}c@{}}\textbf{32.23/0.9330}\\ \textbf{28.14/0.8514}\\ \textbf{26.15/0.7956}\end{tabular} \\ \hline
\end{tabular}
\end{adjustbox}

\label{tab:bicubic_M1}
% \vspace{-10pt}
\end{table*}

==> files/tables/channel.tex <==
\begin{table}[t!]
\caption{\small study on combining different pooling layers for $\times4$.}
\vspace{-5pt}
\centering
% \setlength\arrayrulewidth{0.7pt}
\resizebox{\linewidth}{!}{\begin{tabular}{|c|c|ccccc|c|ccc|}
\hline
\multicolumn{11}{c}{Impact of different pooling layers on TFAM} \\ \hline
 \textbf{Pooling}&  & \multicolumn{5}{c|}{\textbf{Channel Unit}} &  & \multicolumn{3}{c|}{\textbf{Positional Unit}} \\ \cline{1-1} \cline{3-7} \cline{9-11}
\small Avg$_p$ &  & \cmark &  & \cmark & \cmark &  &  & \cmark &  & \cmark \\  
\small Max$_p$ &  &  & \cmark & \cmark &  & \cmark &  & & \cmark & \cmark \\ 
\small LP$_p$ &  &  &  &  & \cmark & \cmark&  & --- & --- & --- \\ \hline\hline

% \small Set5 &  & \rule{0pt}{2ex} 
% $\textbf{32.21}$ & \rule{0pt}{2ex} \rule{0pt}{2ex}
% $32.14$ &\rule{0pt}{2ex} \rule{0pt}{2ex}
% $32.18$ &\rule{0pt}{2ex} \rule{0pt}{2ex}
% $32.16$ &\rule{0pt}{2ex} \rule{0pt}{2ex}
% $32.11$ & & 
% $32.25$ &\rule{0pt}{2ex} \rule{0pt}{2ex}
% $32.19$ &\rule{0pt}{2ex} \rule{0pt}{2ex}
% $\textbf{32.28}$ \\ 


\small Set14 &  &
$\textbf{28.57}$ & \rule{0pt}{2ex} \rule{0pt}{2ex}
$28.54$ & \rule{0pt}{2ex} \rule{0pt}{2ex}
$28.52$ & \rule{0pt}{2ex} \rule{0pt}{2ex}
$28.51$ & \rule{0pt}{2ex} \rule{0pt}{2ex}
$28.49$ &  &
$28.59$ & \rule{0pt}{2ex} \rule{0pt}{2ex}
$28.54$ & \rule{0pt}{2ex} \rule{0pt}{2ex}
$\textbf{28.62}$  \\

\small Urban100 &  &
$\textbf{26.11}$ &\rule{0pt}{2ex} \rule{0pt}{2ex}
$26.08$ &\rule{0pt}{2ex} \rule{0pt}{2ex}
$26.10$ &\rule{0pt}{2ex} \rule{0pt}{2ex}
$26.07$ &\rule{0pt}{2ex} \rule{0pt}{2ex}
$26.01$ &  &
$26.13$ & \rule{0pt}{2ex} \rule{0pt}{2ex}
$26.06$ &\rule{0pt}{2ex} \rule{0pt}{2ex}
$\textbf{26.15}$  \\ \cline{1-1} \cline{3-7} \cline{9-11}  \hline
\end{tabular}}
% \vspace{5pt}

\label{tab:pooling}
% \vspace{-15pt}
\end{table}

% \small Set14 &  & $\textbf{28.57}$ & $28.54$ & $28.52$ & $28.51$ & $28.49$ &  & $28.59$ & $28.54$ & $\textbf{28.62}$  \\ \cline{1-1} \cline{3-7} \cline{9-11}  \hline
% \small B100 &  & $\textbf{27.55}$ & $27.52$ & $27.51$ & $27.50$ & $27.47$ &  & $27.57$ & $27.53$ & $\textbf{27.60}$  \\ \cline{1-1} \cline{3-7} \cline{9-11}  \hline

==> files/tables/inference.tex <==
\begin{table}[htb!]
\centering
\caption{Average Inference Time (s) and Memory Consumption (MB) comparisons with other SOTA models on Urban100 for scale factor $\times4$.}
% \setlength\arrayrulewidth{0.8pt}
\scalebox{0.9}{\begin{tabular}{|c|cccc|}
\hline
\textbf{Model} & \textbf{Params.} & \textbf{Time} & \textbf{Memory} & \textbf{PSNR} \\ \hline \hline
MemNet & $667K$ & $0.543$ & $3,170$ & $25.54$ \\
SRFBN-S& $483K$ & $0.0069$ & $2,960$ & $25.71$ \\
CARN &   $1592K$ & $0.0047$ & $3,015$ & $26.07$ \\
RCAN &   $16000K$ & $0.5927$ & $2,731$ & $26.82$ \\
RDN &    $22000K$ & $0.0294$  & $3,835$ & $26.61$ \\
EDSR &   $43000K$ & $0.0841$ & $8,263$ & $26.64$ \\
\hline
\textbf{MPRNet [Ours]} & $\boldsymbol{538K}$ & $\boldsymbol{0.0095}$  & $\boldsymbol{2,154}$ &  $\boldsymbol{26.31}$ \\ \hline
\end{tabular}}

\label{tab:Inference}
\end{table}

==> files/tables/optim.tex <==
\begin{table}[t!]
\caption{Study of the impact of different optimizer. }
\label{tab:optim}
\centering
% \setlength\arrayrulewidth{0.7pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccc}
\hline
\multicolumn{7}{c}{Performance comparison between Adam and AdamP}                                                                                                              \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Optimizer\\ \hline Scale\end{tabular}}} & \multicolumn{3}{c|}{\textbf{Adam{}}}   & \multicolumn{3}{c|}{\textbf{AdamP{\cite{heo2020slowing}}}}  \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                                                                               & $\times2$    & $\times3$    & \multicolumn{1}{c|}{$\times4$}    & $\times2$    & $\times3$    & \multicolumn{1}{c|}{$\times4$}    \\ \hline
\multicolumn{1}{|l|}{Urban100}                                                                       & 25.44 & 25.44 & \multicolumn{1}{c|}{25.44} & 25.44 & 25.44 & \multicolumn{1}{c|}{25.44} \\ \hline
\end{tabular}}
\end{table}

==> files/tables/params.tex <==
\begin{table}[htb!]

\caption{\small Impact of Depth Multiplier on MPRNet }
\centering
% \setlength\arrayrulewidth{0.5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|cccc|}
\hline

Depth Multiplier & $1.0$ & $0.75$ & $0.5$ & $0.25$ \\ \hline
\# Parameters & $538.2K$ & $470.4K$ & $416.2K$ & $372.7K$  \\ \hline \hline
\small Set114 ($\times4$) & $32.38$ & $32.23$ & $32.01$ & $31.84$ \\ 
\small Urban100 ($\times4$) & $26.31$ & $26.16$ & $25.99$ & $25.83$ \\ \hline
\end{tabular}}
% \end{adjustbox}

\label{tab:NumParams}
\vspace{-15pt}
\end{table}
